Designing for Mobile and Immersive Visual Analytics in the Field

Data collection and analysis in the field is critical for operations in domains such as environmental science and public safety. However, field workers currently face data- and platform-oriented issues in efficient data collection and analysis in the field, such as limited connectivity, screen space, and attentional resources. In this paper, we explore how visual analytics tools might transform field practices by more deeply integrating data into these operations. We use a design probe coupling mobile, cloud and immersive analytics components to guide interviews with ten experts from five domains to explore how visual analytics could support data collection and analysis needs in the field. The results identify shortcomings of current approaches and target scenarios and design considerations for future field analysis systems. We embody these findings in FieldView, an extensible, open-source prototype designed to support critical use cases for situated field analysis. Our findings suggest the potential for integrating mobile and immersive technologies to enhance data's utility for various field operations and new directions for visual analytics tools to transform fieldwork.

==> prose/ds_intro.tex <==
\section{Introduction}

%What's the challenge
Data-oriented decision making is transforming practices in a broad variety of domains. 
%For example, with the substantial number of wildfires in western North America, technology-based solutions for emergency response are receiving considerable attention, including U.S. Congressional support through a 2019 Act to ``promote the use of the best available technology to enhance the effective and cost-efficient response to wildfires'' \cite{dingell2019conservation}.
%DS: I really like the above framing, but it isn't working with the flow---try moving it to the discussion. 
Applications in earth science, geology, and emergency response all leverage data collected in the field to help describe the state of complex environments.
%Field operations in these domains typically rely on a collaboration between people in the field and remote workers in a command central, though current field data analysis efforts focus only on supporting decision making in the command center. 
Field analysts collect data to model the changing state of field sites over time and to share information across teams to increase situational awareness and deepen scientific and operational understanding.
However, current practices for working with data in the field rely heavily on decoupled solutions that separate data analysis from the spatial and temporal contexts that data describes. Data is collected in the field but analyzed elsewhere, such as in operations centers or remote laboratories.
This separation limits analysts' abilities to use this data in on-going operations: remote analysts lack the context and local situational awareness of people in the field, while people in the field lack tools to access, analyze, and act on data while in the field. 
%This work explores the needs, feasibility, and use cases of visualizations in the field.
However, bringing analytics tools into the field creates new design challenges for data analysis systems. This work explores challenges and opportunities for using visualization to support data-driven decision making in the field. 

%What are people doing now
The lack support for analytics in the field means that decision making typically occurs in remote operations centers either during the operation or at a remote site at the end of the operation. 
Current practices for fieldwork require analysts to first preplan their operations based on data from previous collection efforts and archival data streams. Analysts then collect new data either on mobile devices or in field notebooks, physically transport data to a central location to synchronize
with other sources, and replan subsequent collection efforts and operational practices based on the newly revised data.This workflow decontextualizes collected data from the environment, prevents analysts in time-critical situations from reacting to new data, and obscures possible errors in data collection by creating spatial and temporal gaps between data collection and analysis (Fig. \ref{fig:SpatialTemporal}).
%These challenges are exacerbated when data comes from multiple sources: analysts have limited access to additional data collected from other field teams or independent sensors.
%As a result, field operations are plagued by issues caused by both  spatial and temporal gaps between data collection and data analysis 
Spatial gaps in understanding arise when remote analysts lack the physical context 
%of the data collected that field workers do, 
surrounding field data, resulting in a lack of visual grounding for remote analysis and a lack of shared context during real-time operations. 
%a lack of visual grounding to communications from the command center to the field, and unreliable connectivity in remote areas.
%rely on verbal transmissions to ground remote collaborative decision making, or .
Temporal gaps stem from an inability to analyze data during an operation, resulting in stale data being used in dynamic environments, an inability to make timely decisions, and the potential to jeopardize a day's work or even the entire operation due to data quality issues and reduced global awareness of the state of the broader operations.

%Advances in mobile visualization tools \todo{citation} may help bridge the spatial and temporal gaps between data collection and analysis in fieldwork. However, field operations introduce new design challenges not addressed by conventional visualization approaches.  
%In designing visualization systems to the constraints onf field operations, we first need to consider the decision making needs while in the field.
%Though a lab or command central is better suited to the global view of the operation on a desktop computer, the field is better suited to make decisions on lower level tasks while out in the field.
%For example, analysts often need to n dynamic, mobile environments, field analysts must be able to make quick sense of the data alongside its physical context in real time and update their operational plans accordingly.
%Being in the field collecting data, field workers also have the opportunity to visualize data within its spatial context.

We explore how mobile and immersive technologies can help bridge spatial and temporal gaps between data collection and analysis in fieldwork. Specifically,
we examine how coupling these technologies might increase contextual and situational awareness in field analysis practices in order to improve data collection, sharing, analysis, and decision making by better connecting field analysts with their
data. 
Mobile technologies offer portable connectivity to access and synchronize data while in the field and can offer at-a-glance overviews that may help summarize current state of the operation.\todo{cite Brehmer's mobile vis paper from VIS last year} However, mobile technologies suffer from several limitations that may prove challenging for field use. For example, interacting with mobile devices is challenging while wearing gloves and forces analysts to divide their attention between the visualization and environment. Immersive visualization techniques can resolve these issues by visually embedding data in the visual environment \todo{cite situated analysis paper}; however, we have limited insight into how to design effective augmented reality visualizations. Our goal in this paper is to elicit insight into how visualization tools can be designed to effectively support the needs of field data analysis to provide preliminary steps towards a deeper integration of data into field operations. 
%We focus on how mobile data collection, cloud fusion, and augmented reality (AR) visualizations may enable analysts to visualize data as it is collected, allowing analysts to integrate contextual information about the immediate environment into data interpretation. 
%Our approach fuses data from multiple sources to provide field analysts with access to new and existing data from other teams in the field, archival sources, and autonomous sensors. Analysts can then leverage at-a-glance mobile visualizations or immersive interactive visualizations to develop new hypotheses, identify potential errors or gaps in coverage, and adapt operational practices while in the field.

This paper presents an exploratory investigation into how visualization tools could support increased situated awareness and optimize data-driven decision making in the field.
Building on preliminary conversations with field workers in domains ranging from ecology to emergency response, we created an interactive design probe architected to support an integrated data collection and visual analysis workflow through a combination of mobile and immersive visualization tools. 
We use this probe to elicit formal recommendations for visual analytics tools for field work and develop a preliminary prototype based on these recommendations and three target scenarios identified during the interviews where a lack of access to field data causes significant operational challenges. Our results suggest new opportunities for leveraging visualization to empower field operations through data. 
%We seek to identify important decisions better suited to be made in the field than a lab or operations center, what data would enable this decision-making, and how visual analytics systems could support field workers.

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{SpatialTemporal}
	\caption{Temporal and spatial gaps hindering decision making in the field. The temporal gap is characterized by an inability to make decisions until after concluding operations in the field. The spatial gap refers to challenges introduced by removing collected data from the physical environment, reducing local situational awareness during decision making.}
	\label{fig:SpatialTemporal}
\end{figure}

\textbf{Contributions: }\begin{comment} We introduce a novel field data collection and analysis workflow 
%focused on enabling critical
that enables situated decision-making in the field. 
We conducted interviews with field analysts in domains 
%ranging from 
such as environmental science and aerial firefighting to understand limitations in current field data use and synthesize critical design requirements for 
%providing field workers with 
real-time data analysis tools. 
We implement these requirements in %two iterations of user-centered design.
an extensible prototype 
%platform 
leveraging commodity technologies to support field analysis. 
%Our prototype build on prior field data collection systems based on a survey of field analysts in domains ranging from environmental science to aerial firefighting. 
%We leverage immersive visualizations to improve sensemaking in the field for scenarios not well served by conventional mobile technologies.
Building on scenarios identified by analysts, we ground our prototype in three use cases 
%introduce novel visualizations and workflows that 
demonstrating how our 
%situated analytics 
approach may address limitations in field analysis to increase operational efficiency.
\end{comment}
We establish preliminary design considerations and constraints for integrated data collection and analysis tools in the field.
%, summarized in Fig. \ref{fig:teaser}.
We first worked with scientists and public safety officials to identify challenges in current field data practices. 
We use these limitations to develop a design probe demonstrating how mobile and immersive technologies might overcome these limitations.
 We use this probe to scaffold interviews with 10 domain experts about the potential of complimentary mobile and immersive visualizations to transform field operations.
After synthesizing these interviews, we refined the workflow introduced in the design probe to develop FieldView, an open-source prototype system to address use cases inspired by common themes and scenarios identified by analysts (Figure \ref{fig:teaser}).


\begin{comment}

%\todo{DS: Update title to focus on novel components--maybe more abt coupling mobile and immersive vis}
%\begin{figure}
%	\includegraphics[width=\linewidth]{conceptual_figure}
%	\caption{ FieldView enables analysts to collect and explore data fused across various sources within the contexts that data describes to support improved situated data analytics and decision making. \ds{\textbf{update}}}
%\end{figure}
%\todo{DS: Since we have more time, worth using actual images stitched together from system on top of an image of people using it}
\section{Introduction}
Data-oriented decision making is transforming practices in a broad variety of domains. Applications in earth science, geology, and emergency response all leverage data collected in the field to help describe the state of complex environments. 
Quantifying these environments allows analysts to model the changing state of the world over time and to share information across teams to increase situational awareness and deepen scientific and operational understanding. 
However, current practices for working with data in the field rely heavily on decoupled solutions that separate data analysis from the spatial and temporal contexts that data describes: data is collected in the field but analyzed elsewhere, such as in operations centers or remote laboratories.
This separation can limit field analysts' abilities to integrate current data into analysis and decision making practices, introducing significant time and efficiency costs. 

We address this challenge by exploring how mobile and immersive technologies can help bridge spatial and temporal gaps between data collection and analysis in fieldwork. Specifically, we explore how we can couple these technologies to increase contextual and situational awareness in field analysis practices in order to improve data collection, sharing, analysis decision making with relevant visualizations. We focus on how mobile data collection, cloud storage and fusion, mobile device visualizations, and augmented reality (AR) visualizations enable analysts to visualize data as it is collected in order to integrate contextual information about the immediate environment into data interpretation and operational planning.
%adjustments to preplanning. 
%increasing situational awareness through 
Our approach fuses data from multiple sources to provide field analysts with access to new and existing data from other teams in the field and archival sources.
%, and autonomous sensors. 
Analysts can then leverage at-a-glance mobile visualizations and detailed immersive interactive visualizations to develop new hypotheses, identify potential errors or gaps in coverage, and adapt operational practices while in the field.
% increased contextual awareness and situational awareness in data analysis. \todo{unpack this a bit}

%Not covered
Current practices for fieldwork require analysts to first preplan their operations based on archival data from both previous collection efforts and archival data streams.
%Covered
Analysts then collect new data either on mobile devices or in field notebooks, physically transport data to a central location to synchronize with other sources, and replan subsequent collection efforts and operational practices based on the newly revised data. 
%Covered
This workflow decontextualizes collected data from the environment, prevents analysts in time-critical situations from reacting to new data, and obscures possible errors in data collection. 
%Not Covered
These challenges are exacerbated when data comes from multiple sources: analysts have limited access to additional data collected from other field teams or independent sensors. 
%Covered
Our proposed workflow leverages cloud datastores to integrate data from multiple sources as data becomes available, leveraging both local and global data storage to overcome connectivity limitations in the field.
We additionally extend existing practices for field data analysis by allowing analysts to conduct rapid inference using mobile visualizations or immersive embedded visualizations that contextualize data within the physical environment and leverage visual context to support nuanced analyses.
% account for variations in connectivity that may delay synchronization.
% A little covered in the last sentence
%Using these datastores, analysts can gather at-a-glance access to this data through mobile visualizations or access rich interactive visualizations through immersive analysis, increasing the effective screenspace and blending collected data into the immediate environment. 
%Not Covered
This workflow increases contextual awareness to improve data-oriented operational goals, provide real time data quality assessment, and support synchronous operations between field teams. 
%\todo{I don't think this flows well right now :-/}
%field analysts, systems need to retain simplicity, fuse data from multiple sources, enable collaborative analysis, 
%Needs of the problem: simplicity, fusion from multiple sources, collaboration over increased situational awareness, integration of contextual awareness. 

%Address this by AR, focus on field analysts who don't have access to the same view as the ops centers but this approach can support operational centers, increase SA, CA, TTD
%\todo[inline] {DS: Worth calling out in this paragraph what our specific contributions are at a high level (even though it's spelled out in detail below)}
We implement and evaluate this approach in FieldView, an extensible mobile data collection and visualization \ds{prototype} %\todo{wc might matter here?} 
designed to bridge the spatial and temporal gaps between data collection and analysis in the field. 
We developed FieldView in collaboration with field analysts in domains ranging from forest ecology to public safety. 
We discuss how our approach addresses several challenges in field analysis and refine our approach 
%to accommodate field analysis 
using observations from ten domain experts. We demonstrate our approach using three scenarios for field analysis inspired by our discussions with field analysts and unsupported by existing systems: data-mediated teaming, data quality verification, and %on-demand visual 
fusion with autonomous sensors. By coupling mobile data collection and immersive analytics, our approach can foster improved data collection, interpretation, and decision making by providing field analysts with increased access to incoming data and allowing analysts to interpret that data with respect to aspects of the environment only available in the field. 

%\todo[inline]{DS: Based on UIST feedback, also worth noting the design requirements enumeration. MW: Addressed}
\textbf{Contributions: } We introduce a novel field data collection and analysis workflow 
%focused on enabling critical
\ds{that enables situated} decision-making in the field. 
We conducted interviews with field analysts in domains 
%ranging from 
\ds{such as} environmental science and aerial firefighting to understand limitations in current field data use and synthesize critical design requirements for 
%providing field workers with 
real-time data analysis tools. 
We implement \ds{these requirements} in %two iterations of user-centered design.
an extensible prototype 
%platform 
leveraging commodity technologies to support field analysis. 
%Our prototype build on prior field data collection systems based on a survey of field analysts in domains ranging from environmental science to aerial firefighting. 
%We leverage immersive visualizations to improve sensemaking in the field for scenarios not well served by conventional mobile technologies.
Building on scenarios identified by analysts, we ground our prototype in three use cases 
%introduce novel visualizations and workflows that 
demonstrating how our 
%situated analytics 
approach \ds{may} address limitations in field analysis to increase operational efficiency.

%\todo{close on contribution} 
%Our system leverages the portability and growing computational and display power of mobile devices coupled with developments in augmented reality to provide a portable system. 


%Field data collection and emergency response are highly dynamic fields in which a successful operation hinges upon the ability to make strategic decisions in the field.
%Though field workers generally have an understanding of the goals and strategies from preplanning and the ability to make inference based on what they see throughout the day, their decisions are generally not driven by an updated model of the data collected.
%These data-driven decisions are generally reserved for workers in remote operations centers, due to their global view of the data and quality visualization technology at their disposal.
%However, in situations where decisions must be made in a matter of seconds, when there is no connectivity to communication with remote operators, or where being immersed in the situation is critical to decision making, these field workers should be empowered with data and visualizations that allow them to effectively do their jobs.

%Field workers currently have unaddressed needs that can be solved with the right technology.
%As data flows in throughout the day, they do not have the tools to get an idea of what has changed or where preplanning has fallen short.
%Some of this is due to data inundation--where there is so much data flowing in that they cannot efficiently make sense of the data in such a way that does not interfere with the tasks at hand.
%Compounding this effect is the fact that data sources are getting more numerous and heterogeneous.
%More advanced sensing and networking hardware is providing the ability to collect data more efficiently and a more robust view of the environment.
%However, this further contributes to data inundation that causes field workers to largely ignore any synthesized view of the data until they return to a desktop computer where they have the means to make sense of all this data.

%With effective visualization technology in the field, this does not need to be the case.
%We as humans are able to quickly make sense of the our environment so to simply augment that environment with simple, situated visualizations would allow for the quick efficient understanding of the updated data model that field workers currently do not have.
%This is not a complete replacement of the remote operators--their global view of the situation cannot be replicated in the field.
%However, with the right technology given to field workers, they can make the snap decisions and decisions on allocating resources to local goals in ways not previously possible.
%With FieldView, we provide some insight on what specific needs field workers have for data collection and visualization in the field and propose a prototype solution for addressing some existing pain points in the field work process.

%With effective visualization tools of varying aspects of the situation and a global view of the problem without being physically entrenched in any one aspect, these remote operators are well suited to provide information to constituent sub-teams.
%Workers in the field, on the other hand, have an implicit understanding of their physical surroundings that they subconsciously consider when making snap decisions in the field.
%With this work we explore the decisions that are made and could be made in the field, and evaluate the potential for novel technologies to enable data driven decision-making in the field.

%Abowd defines situational awareness as the ability to understand objects, where they are spatially and how their states change over time \todo{UPDATE WITH the 1995 SA Model paper}. 
%This is particularly important for information visualization in areas such as search and rescue [cite], wildfire management [cite] and earth science [cite]. 
%These particular domains share important characteristics: as data is collected in the field, the context updates, and future decisions hinge on an updated interpretation of the new context. 

%Work has been done in exploring how fieldworkers deal with updated data to communicate updated goals from a vantage point of greater situational awareness \textemdash\  a remote operation center. 
%With this work, we seek to also empower the data collectors with updated situational awareness using a workflow that enables local team coordination through visualization of context-aware data in the field. 
%We propose that augmented reality is a good candidate for delivering these types of visualizations, because the projection of data in the real world can leverage our inherent understanding of real-world context.

%We begin by referencing prior work on concepts such as context-aware computing and situational awareness, as well as how these concepts have been used for workflows of data collection to visualization to analysis to decision making. 
%To illustrate the potential for augmented reality in this workflow and facilitate a discussion about its potential, we created a prototype workflow for data entry on a mobile device and augmented reality data visualization. 
%We use a semi-structured interview to evaluate the needs of field researchers and find that many of the pain points that related works have identified are replicated with local domain experts we interviewed. 
%We then use our grounding in related work and interviews with collaborators to propose some design guidelines to enable situational awareness in fieldwork.
%We provide some design guidelines to address salient pain points in the field data collection, visualization and analysis pipeline.
%We then iterate our design by implementing three example use case(s) of the proposed design guidelines that we draw directly from our interviews with field researchers and our design considerations.

\end{comment}

==> prose/introduction.tex <==
\section{Introduction}

Data-oriented decision making is transforming practices in a broad variety of domains. 
For example, with the substantial number of wildfires in western North America, technology-based solutions for emergency response are receiving considerable attention, including U.S. Congressional support through a 2019 Act to ``promote the use of the best available technology to enhance the effective and cost-efficient response to wildfires'' \cite{dingell2019conservation}.
Applications in earth science, geology, and emergency response all leverage data collected in the field to help describe the state of complex environments.
Field operations in these domains typically rely on a collaboration between people in the field and remote workers in a command central, though current field data analysis efforts focus only on supporting decision making in the command center. 
This limits analysts' abilities to use this data in on-going operations: analysts in the command center lack the context and local situational awareness of people in the field, while people in the field lack tools to access, analyze, and act on data while in the field. 
This work explores the needs, feasibility, and use cases of visualizations in the field.

Due to the lack support for analytics in the field, decision making typically occurs in remote operations center either during the operation or at a remote site at the end of the operation. 
For this reason, field operations are plagued by issues caused by both  spatial and temporal gaps between data collection and data analysis (Fig. \ref{fig:SpatialTemporal}).
Spatial gaps in understanding arise due to remote operators not having the physical context of the data collected that field workers do, lack of visual grounding to communications from the command center to the field and unreliable connectivity in remote areas.
Temporal gaps stemming from an inability to analyze data until back in a lab result in field operation on stale data in dynamic environments, an inability to make timely decisions, and could jeapordize a day's work or even the entire operation.

In designing visualization systems to the constraints onf field operations, we first need to consider the decision making needs while in the field.
Though a lab or command central is better suited to the global view of the operation on a desktop computer, the field is better suited to make decisions on lower level tasks while out in the field.
That is, field workers can make quick sense of the data alongside its physical context in real time and update plans accordingly.
Being in the field collecting data, field workers also have the opportunity to visualize data within its spatial context.
This paper focuses on the requirements of solutions that could support this situated awareness to optimize decision making in the field.
Building on preliminary conversations with field workers, we created an interactive design probe architected to support an integrated data collection and visual analysis workflow through a combination of mobile and immersive visual analytics tools. 
We use this probe to elicit formal recommendations for visual analytics tools for field work and develop a preliminary prototype based on these recommendations. 
We seek to identify important decisions better suited to be made in the field than a lab or operations center, what data would enable this decision-making, and how visual analytics systems could support field workers.

\begin{figure}[t]
	\centering
	\includegraphics[width=\columnwidth]{SpatialTemporal}
	\caption{Temporal and spatial gaps hindering decision making in the field. The temporal gap is characterized by an inability to make decisions until after concluding operations in the field. The spatial gap refers to challenges introduced by removing collected data from the physical environment, reducing local situational awareness during decision making.}
	\label{fig:SpatialTemporal}
\end{figure}

\textbf{Contributions: }\begin{comment} We introduce a novel field data collection and analysis workflow 
%focused on enabling critical
that enables situated decision-making in the field. 
We conducted interviews with field analysts in domains 
%ranging from 
such as environmental science and aerial firefighting to understand limitations in current field data use and synthesize critical design requirements for 
%providing field workers with 
real-time data analysis tools. 
We implement these requirements in %two iterations of user-centered design.
an extensible prototype 
%platform 
leveraging commodity technologies to support field analysis. 
%Our prototype build on prior field data collection systems based on a survey of field analysts in domains ranging from environmental science to aerial firefighting. 
%We leverage immersive visualizations to improve sensemaking in the field for scenarios not well served by conventional mobile technologies.
Building on scenarios identified by analysts, we ground our prototype in three use cases 
%introduce novel visualizations and workflows that 
demonstrating how our 
%situated analytics 
approach may address limitations in field analysis to increase operational efficiency.
\end{comment}
We conduct a series of interviews to establish some design considerations and constraints for integrated data collection and analysis tools in the field, summarized in Fig. \ref{fig:teaser}.
We first worked with scientists and public safety officials to identify challenges in current field data practices. 
We use these limitations to develop a design probe demonstrating how mobile and immersive technologies might overcome these limitations.
Using a design probe, we interviewed 10 domain experts about the potential of complimentary mobile and immersive visualizations to transform field operations.
After synthesizing these interviews, we refined the workflow introduced in the design probe to develop FieldView, an open-source prototype system to address use cases inspired by common themes and scenarios identified by analysts.


\begin{comment}

%\todo{DS: Update title to focus on novel components--maybe more abt coupling mobile and immersive vis}
%\begin{figure}
%	\includegraphics[width=\linewidth]{conceptual_figure}
%	\caption{ FieldView enables analysts to collect and explore data fused across various sources within the contexts that data describes to support improved situated data analytics and decision making. \ds{\textbf{update}}}
%\end{figure}
%\todo{DS: Since we have more time, worth using actual images stitched together from system on top of an image of people using it}
\section{Introduction}
Data-oriented decision making is transforming practices in a broad variety of domains. Applications in earth science, geology, and emergency response all leverage data collected in the field to help describe the state of complex environments. 
Quantifying these environments allows analysts to model the changing state of the world over time and to share information across teams to increase situational awareness and deepen scientific and operational understanding. 
However, current practices for working with data in the field rely heavily on decoupled solutions that separate data analysis from the spatial and temporal contexts that data describes: data is collected in the field but analyzed elsewhere, such as in operations centers or remote laboratories.
This separation can limit field analysts' abilities to integrate current data into analysis and decision making practices, introducing significant time and efficiency costs. 

We address this challenge by exploring how mobile and immersive technologies can help bridge spatial and temporal gaps between data collection and analysis in fieldwork. Specifically, we explore how we can couple these technologies to increase contextual and situational awareness in field analysis practices in order to improve data collection, sharing, analysis decision making with relevant visualizations. We focus on how mobile data collection, cloud storage and fusion, mobile device visualizations, and augmented reality (AR) visualizations enable analysts to visualize data as it is collected in order to integrate contextual information about the immediate environment into data interpretation and operational planning.
%adjustments to preplanning. 
%increasing situational awareness through 
Our approach fuses data from multiple sources to provide field analysts with access to new and existing data from other teams in the field and archival sources.
%, and autonomous sensors. 
Analysts can then leverage at-a-glance mobile visualizations and detailed immersive interactive visualizations to develop new hypotheses, identify potential errors or gaps in coverage, and adapt operational practices while in the field.
% increased contextual awareness and situational awareness in data analysis. \todo{unpack this a bit}

%Not covered
Current practices for fieldwork require analysts to first preplan their operations based on archival data from both previous collection efforts and archival data streams.
%Covered
Analysts then collect new data either on mobile devices or in field notebooks, physically transport data to a central location to synchronize with other sources, and replan subsequent collection efforts and operational practices based on the newly revised data. 
%Covered
This workflow decontextualizes collected data from the environment, prevents analysts in time-critical situations from reacting to new data, and obscures possible errors in data collection. 
%Not Covered
These challenges are exacerbated when data comes from multiple sources: analysts have limited access to additional data collected from other field teams or independent sensors. 
%Covered
Our proposed workflow leverages cloud datastores to integrate data from multiple sources as data becomes available, leveraging both local and global data storage to overcome connectivity limitations in the field.
We additionally extend existing practices for field data analysis by allowing analysts to conduct rapid inference using mobile visualizations or immersive embedded visualizations that contextualize data within the physical environment and leverage visual context to support nuanced analyses.
% account for variations in connectivity that may delay synchronization.
% A little covered in the last sentence
%Using these datastores, analysts can gather at-a-glance access to this data through mobile visualizations or access rich interactive visualizations through immersive analysis, increasing the effective screenspace and blending collected data into the immediate environment. 
%Not Covered
This workflow increases contextual awareness to improve data-oriented operational goals, provide real time data quality assessment, and support synchronous operations between field teams. 
%\todo{I don't think this flows well right now :-/}
%field analysts, systems need to retain simplicity, fuse data from multiple sources, enable collaborative analysis, 
%Needs of the problem: simplicity, fusion from multiple sources, collaboration over increased situational awareness, integration of contextual awareness. 

%Address this by AR, focus on field analysts who don't have access to the same view as the ops centers but this approach can support operational centers, increase SA, CA, TTD
%\todo[inline] {DS: Worth calling out in this paragraph what our specific contributions are at a high level (even though it's spelled out in detail below)}
We implement and evaluate this approach in FieldView, an extensible mobile data collection and visualization \ds{prototype} %\todo{wc might matter here?} 
designed to bridge the spatial and temporal gaps between data collection and analysis in the field. 
We developed FieldView in collaboration with field analysts in domains ranging from forest ecology to public safety. 
We discuss how our approach addresses several challenges in field analysis and refine our approach 
%to accommodate field analysis 
using observations from ten domain experts. We demonstrate our approach using three scenarios for field analysis inspired by our discussions with field analysts and unsupported by existing systems: data-mediated teaming, data quality verification, and %on-demand visual 
fusion with autonomous sensors. By coupling mobile data collection and immersive analytics, our approach can foster improved data collection, interpretation, and decision making by providing field analysts with increased access to incoming data and allowing analysts to interpret that data with respect to aspects of the environment only available in the field. 

%\todo[inline]{DS: Based on UIST feedback, also worth noting the design requirements enumeration. MW: Addressed}
\textbf{Contributions: } We introduce a novel field data collection and analysis workflow 
%focused on enabling critical
\ds{that enables situated} decision-making in the field. 
We conducted interviews with field analysts in domains 
%ranging from 
\ds{such as} environmental science and aerial firefighting to understand limitations in current field data use and synthesize critical design requirements for 
%providing field workers with 
real-time data analysis tools. 
We implement \ds{these requirements} in %two iterations of user-centered design.
an extensible prototype 
%platform 
leveraging commodity technologies to support field analysis. 
%Our prototype build on prior field data collection systems based on a survey of field analysts in domains ranging from environmental science to aerial firefighting. 
%We leverage immersive visualizations to improve sensemaking in the field for scenarios not well served by conventional mobile technologies.
Building on scenarios identified by analysts, we ground our prototype in three use cases 
%introduce novel visualizations and workflows that 
demonstrating how our 
%situated analytics 
approach \ds{may} address limitations in field analysis to increase operational efficiency.

%\todo{close on contribution} 
%Our system leverages the portability and growing computational and display power of mobile devices coupled with developments in augmented reality to provide a portable system. 


%Field data collection and emergency response are highly dynamic fields in which a successful operation hinges upon the ability to make strategic decisions in the field.
%Though field workers generally have an understanding of the goals and strategies from preplanning and the ability to make inference based on what they see throughout the day, their decisions are generally not driven by an updated model of the data collected.
%These data-driven decisions are generally reserved for workers in remote operations centers, due to their global view of the data and quality visualization technology at their disposal.
%However, in situations where decisions must be made in a matter of seconds, when there is no connectivity to communication with remote operators, or where being immersed in the situation is critical to decision making, these field workers should be empowered with data and visualizations that allow them to effectively do their jobs.

%Field workers currently have unaddressed needs that can be solved with the right technology.
%As data flows in throughout the day, they do not have the tools to get an idea of what has changed or where preplanning has fallen short.
%Some of this is due to data inundation--where there is so much data flowing in that they cannot efficiently make sense of the data in such a way that does not interfere with the tasks at hand.
%Compounding this effect is the fact that data sources are getting more numerous and heterogeneous.
%More advanced sensing and networking hardware is providing the ability to collect data more efficiently and a more robust view of the environment.
%However, this further contributes to data inundation that causes field workers to largely ignore any synthesized view of the data until they return to a desktop computer where they have the means to make sense of all this data.

%With effective visualization technology in the field, this does not need to be the case.
%We as humans are able to quickly make sense of the our environment so to simply augment that environment with simple, situated visualizations would allow for the quick efficient understanding of the updated data model that field workers currently do not have.
%This is not a complete replacement of the remote operators--their global view of the situation cannot be replicated in the field.
%However, with the right technology given to field workers, they can make the snap decisions and decisions on allocating resources to local goals in ways not previously possible.
%With FieldView, we provide some insight on what specific needs field workers have for data collection and visualization in the field and propose a prototype solution for addressing some existing pain points in the field work process.

%With effective visualization tools of varying aspects of the situation and a global view of the problem without being physically entrenched in any one aspect, these remote operators are well suited to provide information to constituent sub-teams.
%Workers in the field, on the other hand, have an implicit understanding of their physical surroundings that they subconsciously consider when making snap decisions in the field.
%With this work we explore the decisions that are made and could be made in the field, and evaluate the potential for novel technologies to enable data driven decision-making in the field.

%Abowd defines situational awareness as the ability to understand objects, where they are spatially and how their states change over time \todo{UPDATE WITH the 1995 SA Model paper}. 
%This is particularly important for information visualization in areas such as search and rescue [cite], wildfire management [cite] and earth science [cite]. 
%These particular domains share important characteristics: as data is collected in the field, the context updates, and future decisions hinge on an updated interpretation of the new context. 

%Work has been done in exploring how fieldworkers deal with updated data to communicate updated goals from a vantage point of greater situational awareness \textemdash\  a remote operation center. 
%With this work, we seek to also empower the data collectors with updated situational awareness using a workflow that enables local team coordination through visualization of context-aware data in the field. 
%We propose that augmented reality is a good candidate for delivering these types of visualizations, because the projection of data in the real world can leverage our inherent understanding of real-world context.

%We begin by referencing prior work on concepts such as context-aware computing and situational awareness, as well as how these concepts have been used for workflows of data collection to visualization to analysis to decision making. 
%To illustrate the potential for augmented reality in this workflow and facilitate a discussion about its potential, we created a prototype workflow for data entry on a mobile device and augmented reality data visualization. 
%We use a semi-structured interview to evaluate the needs of field researchers and find that many of the pain points that related works have identified are replicated with local domain experts we interviewed. 
%We then use our grounding in related work and interviews with collaborators to propose some design guidelines to enable situational awareness in fieldwork.
%We provide some design guidelines to address salient pain points in the field data collection, visualization and analysis pipeline.
%We then iterate our design by implementing three example use case(s) of the proposed design guidelines that we draw directly from our interviews with field researchers and our design considerations.

\end{comment}
